Fully Sparse 3D Object Detection

As the perception range of LiDAR increases, LiDAR-based 3D object detection becomes a dominant task in the long-range perception task of autonomous driving. The mainstream 3D object detectors usually build dense feature maps in the network backbone and prediction head. However, the computational and spatial costs on the dense feature map are quadratic to the perception range, which makes them hardly scale up to the long-range setting. To enable efficient long-range LiDAR-based object detection, we build a fully sparse 3D object detector (FSD). The computational and spatial cost of FSD is roughly linear to the number of points and independent of the perception range. FSD is built upon the general sparse voxel encoder and a novel sparse instance recognition (SIR) module. SIR first groups the points into instances and then applies instance-wise feature extraction and prediction. In this way, SIR resolves the issue of center feature missing, which hinders the design of the fully sparse architecture for all center-based or anchor-based detectors. Moreover, SIR avoids the time-consuming neighbor queries in previous point-based methods by grouping points into instances. We conduct extensive experiments on the large-scale Waymo Open Dataset to reveal the working mechanism of FSD, and state-of-the-art performance is reported. To demonstrate the superiority of FSD in long-range detection, we also conduct experiments on Argoverse 2 Dataset, which has a much larger perception range ($200m$) than Waymo Open Dataset ($75m$). On such a large perception range, FSD achieves state-of-the-art performance and is 2.4$\times$ faster than the dense counterpart. Codes will be released at https://github.com/TuSimple/SST.

==> abstract.tex <==
As the perception range of LiDAR increases, LiDAR-based 3D object detection becomes a dominant task in the long-range perception task of autonomous driving.
The mainstream 3D object detectors usually build dense feature maps in the network backbone and prediction head.
However, the computational and spatial costs on the dense feature map are quadratic to the perception range, which makes them hardly scale up to the long-range setting.
To enable efficient long-range LiDAR-based object detection, we build a fully sparse 3D object detector (FSD).
The computational and spatial cost of FSD is roughly linear to the number of points and independent of the perception range.
FSD is built upon the general sparse voxel encoder and a novel sparse instance recognition (SIR) module. 
SIR first groups the points into instances and then applies instance-wise feature extraction and prediction.
In this way, SIR resolves the issue of center feature missing, which hinders the design of the fully sparse architecture for all center-based or anchor-based detectors.
Moreover, SIR avoids the time-consuming neighbor queries in previous point-based methods by grouping points into instances.
We conduct extensive experiments on the large-scale Waymo Open Dataset to reveal the working mechanism of FSD, and state-of-the-art performance is reported.
To demonstrate the superiority of FSD in long-range detection, we also conduct experiments on Argoverse 2 Dataset, which has a much larger perception range ($200m$) than Waymo Open Dataset ($75m$). 
On such a large perception range, FSD achieves state-of-the-art performance and is 2.4$\times$ faster than the dense counterpart.
Codes will be released.

==> conclusion.tex <==
\section{Conclusion}
This paper proposes FSD, a fully sparse 3D object detector, aiming for efficient long-range object detection.
FSD utilizes a highly efficient point-based Sparse Instance Recognition module to solve the center feature missing in fully sparse architecture.
FSD achieves not only competitive performance on the widely-used Waymo Open Dataset, but also state-of-the-art performance in the long-range Argoverse 2 dataset with a much faster inference speed than previous detectors.
\mypar{Limitation}
A more elaborately designed grouping strategy may help with performance improvements.
However, it is beyond our design goal in this paper, and we will pursue it in future work.
\mypar{Societal Impacts}
Our method can be deployed in the autonomous driving system. Performance loss caused by improper usage may increase security risks.

==> tables/ped_diff_iou.tex <==
% \begin{table}[ht]

\begin{wraptable}{r}{0.5\columnwidth}
\vspace{-3mm}
\small
\centering
\resizebox{0.49\columnwidth}{!}{
\begin{tabular}{l|cccc}
%   \specialrule{1pt}{0pt}{1pt}
\toprule
Methods & IoU@0.5 & IoU@0.6 & IoU@0.7  & Official $^\ast$\\

\midrule

SST\dag~\cite{sst}  & 71.71 & 49.25 & 17.67 & 71.66 \\
FSD (ours)  & 71.47 & 51.87 & 22.09 & 72.14 \\
\midrule
Improvements  & \down{0.24} & \up{2.62} & \up{4.40} & \up{0.52} \\

\bottomrule
%   \specialrule{1pt}{1pt}{0pt}
\end{tabular}
}
% \vspace{3mm}
\caption{
    Performances of pedestrian detection under different IoU threshold, evaluated with our customized COCO-style tool.
    For fair comparison, we degrade the performance of FSD by early stop, so the two models achieve similar performance with official Waymo metric. 
    $\ast$: Official Waymo level 2 AP (IoU@0.5).
    \dag: Re-implementation using official code.
    }
    \vspace{-4mm}
    \label{tab:ped_diff_iou}

\end{wraptable}


